Reproducible biomarkers: Leveraging nonlinear descriptors in the face of non-ergodicity

Any reliable biomarker has to be specific, generalizable, and reproducible across individuals and contexts. The exact values of such a biomarker must represent similar health states in different individuals and at different times within the same individual to result in the minimum possible false-positive and false-negative rates. The application of standard cut-off points and risk scores across populations hinges upon the assumption of such generalizability. Such generalizability, in turn, hinges upon this condition that the phenomenon investigated by current statistical methods is ergodic, i.e., its statistical measures converge over individuals and time within the finite limit of observations. However, emerging evidence indicates that biological processes abound with non-ergodicity, threatening this generalizability. Here, we present a solution for how to make generalizable inferences by deriving ergodic descriptions of non-ergodic phenomena. For this aim, we proposed capturing the origin of ergodicity-breaking in many biological processes: cascade dynamics. To assess our hypotheses, we embraced the challenge of identifying reliable biomarkers for heart disease and stroke, which, despite being the leading cause of death worldwide and decades of research, lacks reliable biomarkers and risk stratification tools. We showed that raw R-R interval data and its common descriptors based on mean and variance are non-ergodic and non-specific. On the other hand, the cascade-dynamical descriptors, the Hurst exponent encoding linear temporal correlations, and multifractal nonlinearity encoding nonlinear interactions across scales described the non-ergodic heart rate variability ergodically and were specific. This study inaugurates applying the critical concept of ergodicity in discovering and applying digital biomarkers of health and disease.

==> Cover_Letter.tex <==
Dear Editor,
npj Digital Medicine,

I am Madhur Mangalam, a researcher in the Center for Research in Human Movement Variability Department of Biomechanics at the University of Nebraska Omaha, and on behalf of my co-authors, I am excited to submit our manuscript entitled ``Reproducible biomarkers: Leveraging nonlinear descriptors in the face of non-ergodicity'' for publication as a research report in npj Digital Medicine.

Our manuscript delves into the crucial concept of ergodicity and its relevance in biological, medical, and psychological sciences. As life and organisms have unique characteristics, understanding the concept of ergodicity can help uncover patterns that traditional linear models may miss. This is a significant breakthrough as it can provide insights into complex systems and enable us to develop novel disease prevention and treatment approaches.

The reproducibility crisis in science has highlighted the importance of paying due attention to the concept of ergodicity to improve the reproducibility of scientific findings. Our manuscript proposes a novel approach to utilizing digital biomarkers for advancing digital medicine. We found that non-linear descriptors of heart rate variability can be used as effective digital biomarkers, especially in the face of non-ergodicity. This finding is crucial because it enables researchers to use data from individuals and contexts previously deemed unusable, thereby improving the generalizability and reproducibility of scientific findings.

Our team has been studying ergodicity and the reproducibility crisis for several years, and our research can contribute significantly to the scientific community's understanding of these concepts. Our manuscript proposes a new framework for utilizing digital biomarkers, which could have far-reaching implications for digital medicine.

To sum up, our manuscript provides a new approach to utilizing digital biomarkers in the context of non-ergodic systems, which could significantly improve the generalizability and reproducibility of scientific findings.

To ensure the quality and thoroughness of our manuscript, we recommend that Eugene Stanley from Boston University (hes@bu.edu), Frank Harrell from Vanderbilt University (f.harrell@vumc.org), Fred Hasselman from Radboud University (fred.hasselman@ru.nl), Peng Li from Harvard Medical School (pli9@bwh.harvard.edu), and Ralf Metzler from the University of Potsdam (rmetzler@uni-potsdam.de) review our work. Their expertise and insights would be invaluable in evaluating our research’s quality and impact.

In conclusion, we hope that our manuscript meets the standards and requirements of npj Digital Medicine and that it would be a valuable addition to your publication. Thank you for your time and consideration, and we look forward to hearing from you soon.

Sincerely,
Madhur Mangalam
